ExTru: A Lightweight, Fast, and Secure Expirable Trust for the Internet of Things

The resource-constrained nature of the Internet of Things (IoT) devices, poses a challenge in designing a secure, reliable, and particularly high-performance communication for this family of devices. Although side-channel resistant ciphers (either block cipher or stream cipher) are the well-suited solution to establish a guaranteed secure communication, the energy-intensive nature of these ciphers makes them undesirable for particularly lightweight IoT solutions. In this paper, we introduce ExTru, a novel encrypted communication protocol based on stream ciphers that adds a configurable switching & toggling network (CSTN) to not only boost the performance of the communication in lightweight IoT devices, it also consumes far less energy compared with the conventional side-channel resistant ciphers. Although the overall structure of the proposed scheme is leaky against physical attacks, such as side-channel or new scan-based Boolean satisfiability (SAT) attack or algebraic attack, we introduce a dynamic encryption mechanism that removes this vulnerability. We demonstrate how each communicated message in the proposed scheme reduces the level of trust. Accordingly, since a specific number of messages, N, could break the communication and extract the key, by using the dynamic encryption mechanism, ExTru can re-initiate the level of trust periodically after T messages where T<N, to protect the communication against side-channel and scan-based attacks (e.g. SAT attack). Furthermore, we demonstrate that by properly configuring the value of T, ExTru not only increases the strength of security from per "device" to per "message", it also significantly improves energy consumption as well as throughput in comparison with an architecture that only uses a conventional side-channel resistant block/stream cipher.

==> settings.tches.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2569-2925}
\makeatletter
\setDOI{10.13154/tches.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

\setkeys{IACR}{journal=tches}


==> settings.tosc.tex <==
\setfirstpage{0}
\setlastpage{0}
\setvolume{0}
\setnumber{0}

\setISSN{2519-173X}
\makeatletter
\setDOI{10.13154/tosc.v\IACR@vol.i\IACR@no.\IACR@fp-\IACR@lp}
\makeatother

